DexAssist: A Voice-Enabled Dual-LLM Framework for Accessible Web Navigation

Individuals with fine motor impairments, such as those caused by conditions like Parkinson's disease, cerebral palsy, or dyspraxia, face significant challenges in interacting with traditional computer interfaces. Historically, scripted automation has offered some assistance, but these solutions are often too rigid and task-specific, failing to adapt to the diverse needs of users. The advent of Large Language Models (LLMs) promised a more flexible approach, capable of interpreting natural language commands to navigate complex user interfaces. However, current LLMs often misinterpret user intent and have no fallback measures when user instructions do not directly align with the specific wording used in the Document Object Model (DOM). This research presents Dexterity Assist (DexAssist), a dual-LLM system designed to improve the reliability of automated user interface control. Both LLMs work iteratively to ensure successful task execution: the Navigator LLM generates actions based on user input, while the Support LLM assesses the success of these actions and provides continuous feedback based on the DOM content. Our framework displays an increase of ~36 percentage points in overall accuracy within the first iteration of the Support LLM, highlighting its effectiveness in resolving errors in real-time. The main contributions of this paper are the design of a novel dual LLM-based accessibility system, its implementation, and its initial evaluation using 3 e-commerce websites. We conclude by underscoring the potential to build on this framework by optimizing computation time and fine-tuning.

==> methods_testing.tex <==
\section{Methods}

In this study, we designed a dual-Language Model (LLM) system aimed at enhancing the accessibility of web interfaces for users with motor impairments. The system leverages two distinct models: the Navigator LLM, denoted as $\mathcal{N}$, and the Support LLM, denoted as $\mathcal{S}$. The primary role of $\mathcal{N}$ is to process user instructions, represented as $\mathbf{U}$, and translate them into a sequence of executable actions, $\mathbf{A} = \{a_1, a_2, \dots, a_n\}$, where each action $a_i$ is directed at specific elements within the Document Object Model (DOM) of the web page. For example, an action $a_i$ could involve clicking a button or entering text into a form.

The system executes these actions sequentially, monitoring the success of each action through an evaluation function, $\mathcal{E}(a_i)$. Here, $\mathcal{E}(a_i) = 0$ indicates successful execution, while $\mathcal{E}(a_i) \neq 0$ denotes failure. When failures occur, they are aggregated into a set of error codes, $\mathbf{E} = \{\mathcal{E}(a_1), \mathcal{E}(a_2), \dots, \mathcal{E}(a_p)\}$, which reflects the failed attempts by the Navigator LLM to execute certain actions.

To resolve these issues, the Support LLM, $\mathcal{S}$, is activated. This model receives the set $\mathbf{E}$ along with the current DOM structure $\mathbf{D}$ and proposes a revised set of actions $\mathbf{A}' = \{\mathbf{A}'_1, \mathbf{A}'_2, \dots, \mathbf{A}'_g\}$, where each subset $\mathbf{A}'_j$ corresponds to a different error code in $\mathbf{E}$. The system iterates this process up to a maximum of $k=4$ times to ensure task completion. If unresolved errors remain after these iterations, a failure explanation, denoted as $\mathbf{R}$, is returned to the user.

This method ensures that the dual-LLM system can dynamically adapt to the challenges encountered during user interaction, leveraging the collaborative strengths of $\mathcal{N}$ and $\mathcal{S}$ to optimize web accessibility for users with motor impairments.


==> testing_math.tex <==
\subsection{Dual LLM Structure with Error Code Grouping}

The dual-LLM system is designed to handle complex user interactions with web interfaces by employing two distinct language models: the Navigator LLM ($\mathcal{N}$) and the Support LLM ($\mathcal{S}$). This section details the iterative process that occurs when the Navigator LLM encounters execution errors and the Support LLM is engaged to resolve them.

Let $\mathbf{U}$ represent the user instruction, which is processed by the Navigator LLM $\mathcal{N}$ to generate a set of actions $\mathbf{A} = \{a_1, a_2, \dots, a_n\}$, where each $a_i$ is an action corresponding to a DOM element (e.g., clicking a button, typing in a form). The actions are executed sequentially, and the success of each action $a_i$ is determined by evaluating the execution result $\mathcal{E}(a_i)$. Specifically, $\mathcal{E}(a_i) = 0$ indicates success, while $\mathcal{E}(a_i) \neq 0$ indicates failure. These actions are grouped into set $\mathbf{E} = \{\mathcal{E}(a_1), \mathcal{E}(a_2), \dots, \mathcal{E}(a_p)\}$. 

The Support LLM $\mathcal{S}$ is invoked and provided with the set of error codes $\mathbf{E}$ and the DOM structure $\mathcal{D}$. The output from $\mathcal{S}$ is a set of action subsets $\mathbf{A}' = \{\mathbf{A}'_1, \mathbf{A}'_2, \dots, \mathbf{A}'_g\}$, where each subset $\mathbf{A}'_j$ corresponds to one of the error codes $\mathcal{E}(a_i) \in \mathbf{E}$, where $i$ represents any index within the set.

This process can be described in the following steps:

\begin{enumerate}
    \item \textbf{User Instruction:} The user provides an instruction $\mathbf{U}$, which is processed by the Navigator LLM $\mathcal{N}$ to generate a set of actions $\mathbf{A}$.
    \item \textbf{Execution and Error Detection:} Each action $a_i \in \mathbf{A}$ is executed. The system collects any error codes $\mathcal{E}(a_i) \neq 0$ into a set $\mathbf{E}$.
    \item \textbf{Support LLM Invocation:} The Support LLM $\mathcal{S}$ is invoked with the set of error codes $\mathbf{E}$ and the DOM structure $\mathcal{D}$. It returns a set of action subsets $\mathbf{A}' = \{\mathbf{A}'_1, \mathbf{A}'_2, \dots, \mathbf{A}'_g\}$, where each subset $\mathbf{A}'_j$ corresponds to one of the error codes $\mathcal{E}(a_i) \in \mathbf{E}$, where $i$ represents any index within the set.
    \item \textbf{Revised Action Execution:} The Navigator LLM $\mathcal{N}$ revises its action plan based on the suggested action subsets $\mathbf{A}'$ and attempts to execute these new actions.
    \item \textbf{Iteration and Termination:} The process repeats up to a maximum of $k=4$ iterations. If the issue is not resolved after $k$ iterations, the system terminates and returns a final failure explanation to the user.
\end{enumerate}

The iterative sequence can be summarized as follows:
\[
\mathbf{A}_{\text{new}} = \mathcal{N}\left(\mathcal{S}(\mathbf{E}, \mathcal{D})\right)
\]

The mathematical formulation of this process is as follows:

\[
\mathbf{E}_g = \text{Group}(\mathbf{E})
\]

\[
\mathbf{A}' = \mathcal{S}(\mathbf{E}_g, \mathcal{D})
\]

\[
\mathbf{A} \leftarrow \mathbf{A}' 
\]

\[
\text{for } t = 1 \text{ to } k:
\]

\[
\quad \mathbf{A} \leftarrow \mathcal{S}(\mathbf{E}_g, \mathcal{D})
\]

\[
\quad \text{if } \mathcal{E}(\mathbf{A}) = 0: \text{ break}
\]

\noindent
If $\mathcal{E}(\mathbf{A}) \neq 0$ after $k$ iterations, the system returns the final failure explanation $\mathcal{F}$ to the user:

\[
\mathcal{F} = \text{Failure Explanation}
\]

This structured approach, combining the grouping of error codes and iterative action refinement, enhances the efficiency and accuracy of the dual-LLM system in navigating complex web interfaces, particularly for users with accessibility needs.





\subsection{Dual LLM Structure first time}

The dual-LLM system is designed to handle complex user interactions with web interfaces by employing two distinct language models: the Navigator LLM ($\mathcal{N}$) and the Support LLM ($\mathcal{S}$). This section details the iterative process that occurs when the Navigator LLM encounters execution errors and the Support LLM is engaged to resolve them.

Let $\mathbf{U}$ represent the user instruction, which is processed by the Navigator LLM $\mathcal{N}$ to generate a set of actions $\mathbf{A} = \{a_1, a_2, \dots, a_n\}$, where each $a_i$ is an action corresponding to a DOM element (e.g., clicking a button, typing in a form). The actions are executed sequentially, and the success of each action $a_i$ is determined by evaluating the execution result $\mathcal{E}(a_i)$. Specifically, $\mathcal{E}(a_i) = 0$ indicates success, while $\mathcal{E}(a_i) \neq 0$ indicates failure.

If an action $a_i$ fails (i.e., $\mathcal{E}(a_i) \neq 0$), the system invokes the Support LLM $\mathcal{S}$. The Support LLM is provided with the error code $\mathcal{E}(a_i)$ and a structured representation of the DOM elements $\mathcal{D}$ (as described in Section~\ref{sec:dom_structure}). The task of $\mathcal{S}$ is to generate an alternative set of actions $\mathbf{A}' = \{a'_1, a'_2, \dots, a'_m\}$, where $m \leq n$, aimed at resolving the failure encountered by $\mathcal{N}$.

This iterative process can be described as follows:

\begin{enumerate}
    \item \textbf{User Instruction:} $\mathbf{U}$ is provided to $\mathcal{N}$, which generates an initial action set $\mathbf{A}$.
    \item \textbf{Execution and Error Handling:} Each action $a_i \in \mathbf{A}$ is executed. If $\mathcal{E}(a_i) \neq 0$, $\mathcal{S}$ is invoked.
    \item \textbf{Support LLM Response:} $\mathcal{S}$ analyzes $\mathcal{E}(a_i)$ and $\mathcal{D}$ to produce a revised action set $\mathbf{A}'$. For instance, if $\mathcal{N}$ generates an action to \texttt{click 'purchase'} but fails (i.e., the element is not found), $\mathcal{S}$ may suggest \texttt{click 'Add to Cart'} followed by \texttt{click 'Checkout'}.
    \item \textbf{Reiteration:} The Navigator LLM $\mathcal{N}$ revises its action plan based on the suggestions from $\mathcal{S}$ and attempts to execute $\mathbf{A}'$.
    \item \textbf{Termination Condition:} The system allows a maximum of $k=4$ iterations. If the issue is not resolved after $k$ iterations, the process terminates, and the system returns a failure explanation $\mathcal{F}$ to the user, detailing what could not be accomplished.
\end{enumerate}

Mathematically, the iterative process can be formalized as:

\[
\mathbf{A}_{\text{new}} = \mathcal{S}(\mathcal{E}(a_i), \mathcal{D})
\]

\[
\mathbf{A} \leftarrow \mathbf{A}_{\text{new}}
\]

\[
\text{for } t = 1 \text{ to } k:
\]

\[
\quad \mathbf{A} \leftarrow \mathcal{S}(\mathcal{E}(a_i), \mathcal{D})
\]

\[
\quad \text{if } \mathcal{E}(\mathbf{A}) = 0: \text{ break}
\]

\noindent
If $\mathcal{E}(\mathbf{A}) \neq 0$ after $k$ iterations, the system abandons the process and returns a final explanation $\mathcal{F}$ to the user:

\[
\mathcal{F} = \text{Failure Explanation}
\]

This dual-LLM structure, combining $\mathcal{N}$ and $\mathcal{S}$ in an iterative feedback loop, significantly enhances the robustness of user interactions with web interfaces, particularly for users with motor impairments.



\subsection{Dual LLM Third time}

The dual-LLM system is designed to handle complex user interactions with web interfaces by employing two distinct language models: the Navigator LLM ($\mathcal{N}$) and the Support LLM ($\mathcal{S}$). This section details the iterative process that occurs when the Navigator LLM encounters execution errors and the Support LLM is engaged to resolve them.

Let $\mathbf{U}$ represent the user instruction, which is processed by the Navigator LLM $\mathcal{N}$ to generate a set of actions $\mathbf{A} = \{a_1, a_2, \dots, a_n\}$, where each $a_i$ is an action corresponding to a DOM element (e.g., clicking a button, typing in a form). The actions are executed sequentially, and the success of each action $a_i$ is determined by evaluating the execution result $\mathcal{E}(a_i)$. Specifically, $\mathcal{E}(a_i) = 0$ indicates success, while $\mathcal{E}(a_i) \neq 0$ indicates failure.

If an action $a_i$ fails (i.e., $\mathcal{E}(a_i) \neq 0$), the system invokes the Support LLM $\mathcal{S}$. The Support LLM is provided with the error code $\mathcal{E}(a_i)$ and a structured representation of the DOM elements $\mathcal{D}$ (as described in Section~\ref{sec:dom_structure}). The task of $\mathcal{S}$ is to generate an alternative set of actions $\mathbf{A}' = \{a'_1, a'_2, \dots, a'_m\}$, where $m \leq n$, aimed at resolving the failure encountered by $\mathcal{N}$.

This iterative process can be described as follows:

\begin{enumerate}
    \item \textbf{User Instruction:} $\mathbf{U}$ is provided to $\mathcal{N}$, which generates an initial action set $\mathbf{A}$.
    \item \textbf{Execution and Error Handling:} Each action $a_i \in \mathbf{A}$ is executed. If $\mathcal{E}(a_i) \neq 0$, $\mathcal{S}$ is invoked.
    \item \textbf{Support LLM Response:} $\mathcal{S}$ analyzes $\mathcal{E}(a_i)$ and $\mathcal{D}$ to produce a revised action set $\mathbf{A}'$. For instance, if $\mathcal{N}$ generates an action to \texttt{click 'purchase'} but fails (i.e., the element is not found), $\mathcal{S}$ may suggest \texttt{click 'Add to Cart'} followed by \texttt{click 'Checkout'}.
    \item \textbf{Reiteration:} The Navigator LLM $\mathcal{N}$ revises its action plan based on the suggestions from $\mathcal{S}$ and attempts to execute $\mathbf{A}'$.
    \item \textbf{Termination Condition:} The system allows a maximum of $k=4$ iterations. If the issue is not resolved after $k$ iterations, the process terminates, and the system returns a failure explanation $\mathcal{F}$ to the user, detailing what could not be accomplished.
\end{enumerate}

Mathematically, the iterative process can be formalized as:

\[
\mathbf{A}_{\text{new}} = \mathcal{S}(\mathcal{E}(a_i), \mathcal{D})
\]

\[
\mathbf{A} \leftarrow \mathbf{A}_{\text{new}}
\]

\[
\text{for } t = 1 \text{ to } k:
\]

\[
\quad \mathbf{A} \leftarrow \mathcal{S}(\mathcal{E}(a_i), \mathcal{D})
\]

\[
\quad \text{if } \mathcal{E}(\mathbf{A}) = 0: \text{ break}
\]

\noindent
If $\mathcal{E}(\mathbf{A}) \neq 0$ after $k$ iterations, the system abandons the process and returns a final explanation $\mathcal{F}$ to the user:

\[
\mathcal{F} = \text{Failure Explanation}
\]

This dual-LLM structure, combining $\mathcal{N}$ and $\mathcal{S}$ in an iterative feedback loop, significantly enhances the robustness of user interactions with web interfaces, particularly for users with motor impairments.



\subsection{Dual LLM Structure with Error Code Grouping}

The dual-LLM system is designed to handle complex user interactions with web interfaces by utilizing two distinct language models: the Navigator LLM ($\mathcal{N}$) and the Support LLM ($\mathcal{S}$). To optimize error handling and ensure robust performance, the system groups related execution errors together, enabling the Support LLM to address multiple issues simultaneously.

When a user instruction $\mathbf{U}$ is provided, the Navigator LLM $\mathcal{N}$ generates a set of actions $\mathbf{A} = \{a_1, a_2, \dots, a_n\}$, where each action $a_i$ corresponds to an interaction with a specific DOM element. These actions are then executed in sequence. If certain actions fail—due to elements not being found or other execution issues—the system groups these errors and invokes the Support LLM $\mathcal{S}$.

The Support LLM analyzes the grouped errors in conjunction with the DOM structure $\mathcal{D}$ and provides a set of alternative action subsets $\mathbf{A}' = \{\mathbf{A}'_1, \mathbf{A}'_2, \dots, \mathbf{A}'_g\}$, where each subset corresponds to a different aspect of the issues encountered. For example, if the Navigator LLM attempts to click a 'purchase' button that cannot be found, the Support LLM might suggest alternative actions such as \texttt{click 'Add to Cart'} followed by \texttt{click 'Checkout'}.

The revised actions are then executed by the Navigator LLM, and the process may iterate up to $k=4$ times to ensure successful task completion. If the issue remains unresolved after these iterations, the system provides a final explanation $\mathcal{F}$ to the user, detailing what could not be accomplished.

This structured approach allows the dual-LLM system to efficiently manage complex interactions, dynamically adapting to user needs while minimizing errors and improving the overall accessibility of web interfaces.


